An analytic distribution function for a massless cored stellar system in a cuspy dark matter halo

We demonstrate the existence of distribution functions that can be used to represent spherical massless cored stellar systems embedded in cuspy dark matter halos with constant mildly tangential velocity anisotropy. In particular, we derive analytically the functional form of the distribution function for a Plummer stellar sphere in a Hernquist dark halo, for \beta_0 = -0.5 and for different degrees of embedding. This particular example satisfies the condition that the central logarithmic slope of the light profile \gamma_0 > 2 \beta_0. Our models have velocity dispersion profiles similar to those observed in nearby dwarf spheroidal galaxies. Hence they can be used to generate initial conditions for a variety of problems, including N-body simulations that may represent dwarf galaxies in the Local Group.

==> aas_macros.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 4.0.
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package and need to resolve the macro definitions
%  in the BibTeX entries returned by the ADS abstract service.
%
%  If you plan not to use this file to resolve the journal macros
%  rather than the whole AAS TeX macro package, you should save the
%  file as ``aas_macros.sty'' and then include it in your paper by
%  using a construct such as:
%	\documentstyle[11pt,aas_macros]{article}
%
%  For more information on the AASTeX macro package, please see the URL
%	http://www.aas.org/publications/aastex.html
%  For more information about ADS abstract server, please see the URL
%	http://adswww.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).
\newcommand\aj{{AJ}}                   % Astronomical Journal
\newcommand\araa{{ARA\&A}}             % Annual Review of Astron and Astrophys
\newcommand\apj{{ApJ}}                 % Astrophysical Journal
\newcommand\apjl{{ApJ}}                % Astrophysical Journal, Letters
\newcommand\apjs{{ApJS}}               % Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}           % Applied Optics
\newcommand\apss{{Ap\&SS}}             % Astrophysics and Space Science
\newcommand\aap{{A\&A}}                % Astronomy and Astrophysics
\newcommand\aapr{{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}              % Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}                 % Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}               % Bulletin of the AAS
\newcommand\jrasc{{JRASC}}             % Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}            % Memoirs of the RAS
\newcommand\mnras{{MNRAS}}             % Monthly Notices of the RAS
\newcommand\pra{{Phys.~Rev.~A}}        % Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}        % Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}        % Physical Review C
\newcommand\prd{{Phys.~Rev.~D}}        % Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}        % Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}    % Physical Review Letters
\newcommand\pasp{{PASP}}               % Publications of the ASP
\newcommand\pasj{{PASJ}}               % Publications of the ASJ
\newcommand\qjras{{QJRAS}}             % Quarterly Journal of the RAS
\newcommand\skytel{{S\&T}}             % Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}      % Solar Physics
\newcommand\sovast{{Soviet~Ast.}}      % Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}     % Space Science Reviews
\newcommand\zap{{ZAp}}                 % Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}              % Nature
\newcommand\iaucirc{{IAU~Circ.}}       % IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}} % Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}   % Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}   % Physics Reports
\newcommand\physscr{{Phys.~Scr}}   % Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}   % Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}   % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
